Optical Efficiency Measurements of Large Area Luminescent Solar Concentrators

Luminescent solar concentrators (LSCs) are able to concentrate both direct and diffuse solar radiation and this ability has led to great interest in using them to improve solar energy capture when coupled to traditional photovoltaics (PV). In principle, a large area LSC could concentrate light onto a much smaller area of PV, thus reducing costs or enabling new architectures. However, LSCs suffer from various optical losses which are hard to quantify using simple measurements of power conversion efficiency. Here, we show that spatially resolved photoluminescence quantum efficiency measurements on large area LSCs can be used to resolve various losses processes such as out-coupling, self-absorption via emitters and self-absorption from the LSC matrix. Further, these measurements allow for the extrapolation of device performance to arbitrarily large LSCs. Our results provide insight into the optimization of optical properties and guide the design of future LSCs for improved solar energy capture.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
